Variational inference for large Bayesian vector autoregressions

We propose a novel variational Bayes approach to estimate high-dimensional vector autoregression (VAR) models with hierarchical shrinkage priors. Our approach does not rely on a conventional structural VAR representation of the parameter space for posterior inference. Instead, we elicit hierarchical shrinkage priors directly on the matrix of regression coefficients so that (1) the prior structure directly maps into posterior inference on the reduced-form transition matrix, and (2) posterior estimates are more robust to variables permutation. An extensive simulation study provides evidence that our approach compares favourably against existing linear and non-linear Markov Chain Monte Carlo and variational Bayes methods. We investigate both the statistical and economic value of the forecasts from our variational inference approach within the context of a mean-variance investor allocating her wealth in a large set of different industry portfolios. The results show that more accurate estimates translate into substantial statistical and economic out-of-sample gains. The results hold across different hierarchical shrinkage priors and model dimensions.

==> Tables/R2oos.tex <==
\begin{sidewaystable}
\centering
\caption{\bf $R^2_{oos}$ across industries}
\vspace{0.1in}
\begin{justify}
\footnotesize{This table reports a set of descriptive statistics for the $R_{oos}^2$ expressed in \%, across individual industry portfolios. Panel A reports the results for the 49 industry classification, whereas Panel B reports the results for the 30 industry classification. For each case we report the mean and median $R_{oos}^2$ across industries as well as a set of percentiles and the min and max values. In addition, we report the percentage of industry portfolios for which a given model can generate positive out-of-sample $R^2$, i.e., $\text{Prob}\left(R_{oos}^2>0\right)$.}
\end{justify}
\vspace{1em}
\renewcommand{\arraystretch}{1}
\begin{flushleft}
{\bf Panel A: \normalfont $R_{oos}^2$ (\%) for 49 industry portfolios}
\end{flushleft}\vspace{0.1in}
\resizebox{1\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
          & \multicolumn{4}{c}{Univariate} &       & \multicolumn{14}{c}{Multivariate} \\
          \cmidrule{7-20}
          &       &       &       &       &       & \multicolumn{4}{c}{MCMC}      &       & \multicolumn{4}{c}{LVB} &       & \multicolumn{4}{c}{VB} \\
          \cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
          & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} \\
          \midrule 
    Mean  & -30.17 & -15.13 & -5.94 & -15.04 &       & -31.59 & -17.16 & -6.58 & -15.30 &       & -31.38 & -17.16 & -15.80 & -6.22 &       & -23.76 & -5.09 & -4.62 & -3.87 \\
    Median   & -28.23 & -14.13 & -5.31 & -13.97 &       & -28.92 & -16.20 & -5.96 & -14.81 &       & -29.08 & -15.41 & -14.57 & -5.97 &       & -20.84 & -5.52 & -5.17 & -4.08 \\
  [1em]
\multicolumn{1}{l}{Percentile} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{l}{2.5} & -54.67 & -26.40 & -13.00 & -27.89 &       & -60.15 & -32.68 & -14.32 & -29.52 &       & -60.53 & -32.56 & -29.94 & -12.49 &       & -49.95 & -11.24 & -9.30 & -10.22 \\
    \multicolumn{1}{l}{25} & -36.49 & -19.70 & -7.72 & -18.81 &       & -38.58 & -21.46 & -8.54 & -19.33 &       & -38.38 & -21.29 & -20.06 & -8.74 &       & -29.59 & -7.98 & -7.44 & -6.07 \\
    \multicolumn{1}{l}{75} & -22.64 & -11.20 & -3.70 & -11.16 &       & -23.48 & -12.75 & -4.45 & -10.98 &       & -23.42 & -13.31 & -11.63 & -4.08 &       & -17.76 & -2.08 & -1.62 & -1.33 \\
    \multicolumn{1}{l}{97.5} & -13.81 & -5.76 & -0.89 & -5.54 &       & -15.24 & -6.92 & -1.51 & -5.49 &       & -13.14 & -5.89 & -4.91 & 0.75  &       & -9.65 & 1.71  & 1.49  & 1.20 \\
 [1em]
    Min   & -56.74 & -31.41 & -13.10 & -30.55 &       & -60.24 & -33.34 & -15.81 & -32.72 &       & -61.91 & -33.86 & -31.16 & -13.62 &       & -50.91 & -12.51 & -9.34 & -10.31 \\
    Max   & -12.71 & -4.45 & -0.60 & -4.52 &       & -13.86 & -6.60 & -1.48 & -5.08 &       & -11.96 & -5.84 & -4.12 & 0.99  &       & -6.57 & 2.54  & 1.68  & 3.05 \\
    $\text{Prob}\left(R_{oos}^2>0\right)$ & 0.00  & 0.00  & 0.00  & 0.00  &       & 0.00  & 0.00  & 0.00  & 0.00  &       & 0.00  & 0.00  & 0.00  & 4.08  &       & 0.00  & 6.12  & 8.16  & 8.16 \\
    \bottomrule
\end{tabular}}
    
\vspace{1em}
\renewcommand{\arraystretch}{1}
\begin{flushleft}
{\bf Panel B: \normalfont $R_{oos}^2$ (\%) for 30 industry portfolios}
\end{flushleft}\vspace{0.1in}
\resizebox{1\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
          & \multicolumn{4}{c}{Univariate} &       & \multicolumn{14}{c}{Multivariate} \\
         \cmidrule{7-20}
          &       &       &       &       &       & \multicolumn{4}{c}{MCMC}      &       & \multicolumn{4}{c}{LVB} &       & \multicolumn{4}{c}{VB} \\
          \cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
          & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} \\
          \midrule 
    Mean  & -13.22 & -6.38 & -1.47 & -5.45 &       & -13.84 & -6.99 & -2.77 & -5.29 &       & -36.77 & -2.54 & -2.53 & -3.05 &       & -21.22 & -0.59 & -0.65 & -0.53 \\
    Median   & -13.71 & -6.96 & -1.67 & -5.91 &       & -14.67 & -7.38 & -2.97 & -5.48 &       & -31.42 & -2.80 & -2.85 & -3.21 &       & -16.46 & -0.76 & -0.86 & -0.77 \\
  [1em]
\multicolumn{1}{l}{Percentile} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{l}{2.5} & -19.87 & -10.82 & -3.50 & -9.63 &       & -20.58 & -11.46 & -5.78 & -9.06 &       & -101.27 & -4.18 & -4.34 & -5.61 &       & -72.42 & -2.55 & -2.70 & -2.73 \\
    \multicolumn{1}{l}{25} & -15.04 & -7.84 & -2.49 & -6.88 &       & -15.58 & -8.37 & -3.98 & -6.56 &       & -36.23 & -3.56 & -3.43 & -4.10 &       & -23.18 & -1.44 & -1.49 & -1.18 \\
    \multicolumn{1}{l}{75} & -11.09 & -5.04 & -0.47 & -4.13 &       & -11.69 & -5.77 & -1.74 & -4.07 &       & -26.65 & -1.81 & -1.94 & -2.06 &       & -12.52 & 0.48  & 0.22  & 0.34 \\
    \multicolumn{1}{l}{97.5} & -6.27 & -1.79 & 1.55  & -0.94 &       & -6.66 & -2.12 & 1.07  & -0.84 &       & -12.99 & 0.77  & 0.85  & 0.79  &       & -5.24 & 1.86  & 1.63  & 1.53 \\
    [1em]
    Min   & -20.37 & -11.36 & -3.57 & -10.19 &       & -21.10 & -11.78 & -5.95 & -9.50 &       & -108.95 & -4.21 & -4.42 & -5.77 &       & -79.18 & -2.66 & -2.82 & -2.86 \\
    Max   & -5.90 & -1.56 & 1.67  & -0.65 &       & -6.28 & -1.56 & 1.37  & -0.41 &       & -12.35 & 0.81  & 0.90  & 0.97  &       & -4.65 & 1.92  & 1.65  & 1.59 \\
    $\text{Prob}\left(R_{oos}^2>0\right)$ & 0.00  & 0.00  & 13.33 & 0.00  &       & 0.00  & 0.00  & 6.67  & 0.00  &       & 0.00  & 10.00 & 10.00 & 10.00 &       & 0.00  & 33.33 & 30.00 & 33.33 \\
    \bottomrule
    \end{tabular}%
 }
\label{tab:R2oos}
\end{sidewaystable}

==> Tables/R2oos_expansions.tex <==
\begin{sidewaystable}
\centering
\caption{\bf $R^2_{oos}$ across industries during expansions}
\vspace{0.1in}
\begin{justify}
\footnotesize{This table reports a set of descriptive statistics for the sample of cryptocurrency pairs used for the single- and double-sorting strategies. Each month we select the top 100 most liquid cryptocurrency pairs based on the lagged within-month mean of the \cite{amihud2002illiquidity} ratio. The table reports the time-series average of the cross-sectional distribution of the returns, raw trading volume (in \$mln), market capitalization (in \$mln), realised volatility and the \citet{amihud2002illiquidity} ratio. The sample period is from March 1, 2017 to March 1, 2022.}
\end{justify}
\vspace{1em}
\renewcommand{\arraystretch}{1}
\begin{flushleft}
{\bf Panel A: \normalfont $R_{oos}^2$ (\%) for 49 industry portfolios}
\end{flushleft}\vspace{0.1in}
\resizebox{1\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
          & \multicolumn{4}{c}{Univariate} &       & \multicolumn{14}{c}{Multivariate} \\
          \cmidrule{7-20}
          &       &       &       &       &       & \multicolumn{4}{c}{MCMC}      &       & \multicolumn{4}{c}{LVB} &       & \multicolumn{4}{c}{VB} \\
          \cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
          & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} \\
          \midrule 
     Mean  & -31.97 & -14.17 & -4.99 & -15.02 &       & -33.23 & -16.68 & -6.81 & -16.00 &       & -33.04 & -16.29 & -15.50 & -6.25 &       & -25.28 & -7.33 & -6.96 & -5.74 \\
    Median   & -31.00 & -13.45 & -4.78 & -14.14 &       & -31.71 & -15.48 & -6.32 & -14.94 &       & -31.23 & -15.59 & -15.03 & -5.62 &       & -24.13 & -7.89 & -6.61 & -5.53 \\
      [1em]
\multicolumn{1}{l}{Percentile} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{l}{2.5}   & -55.07 & -24.48 & -10.90 & -28.66 &       & -59.60 & -31.69 & -13.70 & -30.60 &       & -56.72 & -34.12 & -30.76 & -13.63 &       & -45.36 & -13.91 & -13.74 & -14.24 \\
    \multicolumn{1}{l}{25}   & -38.58 & -18.14 & -7.12 & -18.13 &       & -39.91 & -20.97 & -9.10 & -20.08 &       & -38.95 & -19.36 & -18.66 & -8.44 &       & -29.34 & -9.99 & -9.25 & -7.56 \\
    \multicolumn{1}{l}{75}   & -25.49 & -10.75 & -3.58 & -11.63 &       & -26.11 & -12.48 & -5.13 & -12.22 &       & -25.85 & -12.11 & -11.72 & -3.96 &       & -19.33 & -4.57 & -4.75 & -3.29 \\
   \multicolumn{1}{l}{97.5}  & -14.02 & -3.48 & 1.95  & -4.32 &       & -15.02 & -5.88 & -0.54 & -5.21 &       & -14.41 & -4.63 & -4.42 & -0.60 &       & -10.04 & -0.91 & -0.50 & -0.59 \\
     [1em]
    Min   & -61.81 & -25.82 & -11.45 & -29.48 &       & -69.54 & -35.54 & -17.21 & -36.07 &       & -70.02 & -38.45 & -33.59 & -15.32 &       & -54.95 & -14.00 & -13.80 & -15.70 \\
    Max   & -6.75 & 0.92  & 2.42  & 0.93  &       & -4.22 & -0.38 & -0.23 & -0.36 &       & -5.31 & -1.10 & -2.30 & 0.43  &       & -7.07 & -0.85 & 1.13  & 0.24 \\
    $\text{Prob}\left(R_{oos}^2>0\right)$ & 0.00  & 2.04  & 4.08  & 2.04  &       & 0.00  & 0.00  & 0.00  & 0.00  &       & 0.00  & 0.00  & 0.00  & 2.04  &       & 0.00  & 0.00  & 2.04  & 2.04 \\
    \bottomrule
\end{tabular}}
    
\vspace{1em}
\renewcommand{\arraystretch}{1}
\begin{flushleft}
{\bf Panel B: \normalfont $R_{oos}^2$ (\%) for 30 industry portfolios}
\end{flushleft}\vspace{0.1in}
\resizebox{1\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
          & \multicolumn{4}{c}{Univariate} &       & \multicolumn{14}{c}{Multivariate} \\
         \cmidrule{7-20}
          &       &       &       &       &       & \multicolumn{4}{c}{MCMC}      &       & \multicolumn{4}{c}{LVB} &       & \multicolumn{4}{c}{VB} \\
          \cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
          & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} \\
          \midrule
        Mean  & -16.97 & -8.54 & -3.17 & -7.61 &       & -17.65 & -9.29 & -4.39 & -7.42 &       & -39.64 & -3.29 & -3.31 & -4.15 &       & -23.68 & -1.36 & -1.43 & -1.34 \\
    Median   & -17.72 & -8.68 & -3.26 & -7.76 &       & -18.37 & -9.38 & -4.32 & -7.65 &       & -33.23 & -3.12 & -3.17 & -4.11 &       & -19.85 & -1.57 & -1.59 & -1.37 \\
       [1em]
\multicolumn{1}{l}{Percentile} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{l}{2.5}   & -24.21 & -13.15 & -5.09 & -12.10 &       & -24.95 & -14.08 & -7.10 & -11.66 &       & -102.95 & -6.25 & -6.09 & -6.84 &       & -74.13 & -2.36 & -2.43 & -2.84 \\
    \multicolumn{1}{l}{25}    & -18.50 & -9.80 & -3.61 & -8.56 &       & -19.45 & -10.54 & -5.36 & -8.52 &       & -45.31 & -4.38 & -4.57 & -5.54 &       & -25.87 & -1.88 & -1.93 & -1.83 \\
    \multicolumn{1}{l}{75}    & -14.01 & -7.26 & -2.43 & -6.68 &       & -14.95 & -7.84 & -3.56 & -6.08 &       & -26.35 & -2.38 & -2.50 & -2.83 &       & -15.81 & -0.89 & -0.98 & -0.99 \\
    \multicolumn{1}{l}{97.5}  & -8.39 & -3.23 & -0.95 & -3.18 &       & -8.86 & -4.17 & -1.58 & -3.17 &       & -13.80 & -0.89 & -0.91 & -1.33 &       & -8.16 & 0.55  & 0.40  & 0.40 \\
          &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    Min   & -24.32 & -13.34 & -5.09 & -12.38 &       & -25.03 & -14.21 & -7.30 & -11.90 &       & -110.92 & -6.67 & -6.48 & -6.84 &       & -80.06 & -2.38 & -2.46 & -3.07 \\
    Max   & -6.77 & -2.61 & -0.95 & -2.82 &       & -7.20 & -3.37 & -1.40 & -2.64 &       & -12.10 & -0.88 & -0.88 & -1.28 &       & -7.47 & 0.64  & 0.40  & 0.43 \\
    $\text{Prob}\left(R_{oos}^2>0\right)$ & 0.00  & 0.00  & 0.00  & 0.00  &       & 0.00  & 0.00  & 0.00  & 0.00  &       & 0.00  & 0.00  & 0.00  & 0.00  &       & 0.00  & 6.67  & 6.67  & 6.67 \\
 
    \bottomrule
    \end{tabular}%
 }
\label{tab:R2oos_expansion}
\end{sidewaystable}

==> Tables/R2oos_recessions.tex <==
\begin{sidewaystable}
\centering
\caption{\bf $R^2_{oos}$ across industries during recessions}
\vspace{0.1in}
\begin{justify}
\footnotesize{This table reports a set of descriptive statistics for the $R_{oos}^2$ calculated during recession periods expressed in \%, across individual industry portfolios. Panel A reports the results for the 49 industry classification, whereas Panel B reports the results for the 30 industry classification. For each case we report the mean and median $R_{oos}^2$ across industries as well as a set of percentiles and the min and max values. In addition, we report the percentage of industry portfolios for which a given model can generate positive out-of-sample $R^2$, i.e., $\text{Prob}\left(R_{oos}^2>0\right)$.}
\end{justify}
\vspace{1em}
\renewcommand{\arraystretch}{1}
\begin{flushleft}
{\bf Panel A: \normalfont $R_{oos}^2$ (\%) for 49 industry portfolios}
\end{flushleft}\vspace{0.1in}
\resizebox{1\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
          & \multicolumn{4}{c}{Univariate} &       & \multicolumn{14}{c}{Multivariate} \\
          \cmidrule{7-20}
          &       &       &       &       &       & \multicolumn{4}{c}{MCMC}      &       & \multicolumn{4}{c}{LVB} &       & \multicolumn{4}{c}{VB} \\
          \cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
          & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} \\
          \midrule 
           Mean  & -30.20 & -19.93 & -9.34 & -17.67 &       & -31.99 & -21.03 & -7.40 & -16.19 &       & -31.55 & -22.19 & -19.15 & -7.67 &       & -24.07 & -0.68 & 0.05  & -0.24 \\
    Median  & -22.36 & -16.31 & -5.97 & -13.44 &       & -24.02 & -17.55 & -4.47 & -12.96 &       & -24.35 & -18.66 & -16.80 & -6.00 &       & -19.29 & 1.36  & 1.60  & 0.61 \\
    [1em]
\multicolumn{1}{l}{Percentile} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{l}{2.5}   & -123.70 & -78.74 & -38.83 & -76.19 &       & -129.91 & -81.34 & -37.73 & -71.35 &       & -142.57 & -89.82 & -82.66 & -40.93 &       & -122.20 & -28.24 & -29.38 & -26.14 \\
     \multicolumn{1}{l}{25}    & -35.34 & -23.74 & -12.55 & -21.37 &       & -36.94 & -26.26 & -10.91 & -21.30 &       & -34.56 & -26.55 & -24.01 & -10.86 &       & -28.18 & -3.66 & -3.35 & -2.26 \\
     \multicolumn{1}{l}{75}    & -13.44 & -8.48 & -2.03 & -7.18 &       & -14.88 & -9.64 & -1.58 & -6.20 &       & -16.39 & -11.73 & -7.41 & -1.33 &       & -9.03 & 5.08  & 6.33  & 3.93 \\
     \multicolumn{1}{l}{97.5}  & 6.12  & 4.34  & 4.31  & 5.54  &       & 5.64  & 5.15  & 6.29  & 6.62  &       & 5.09  & 2.27  & 5.17  & 5.42  &       & 13.83 & 14.23 & 11.30 & 9.99 \\
    [1em]
    Min   & -154.23 & -103.91 & -55.07 & -102.15 &       & -162.39 & -102.52 & -47.76 & -90.60 &       & -159.59 & -100.91 & -90.23 & -47.93 &       & -135.94 & -62.53 & -48.41 & -46.11 \\
    Max   & 10.77 & 4.69  & 6.13  & 6.38  &       & 12.23 & 11.02 & 6.48  & 10.59 &       & 12.41 & 2.92  & 6.68  & 5.82  &       & 15.63 & 14.73 & 14.28 & 11.09 \\
    $\text{Prob}\left(R_{oos}^2>0\right)$ & 6.12  & 6.12  & 12.24 & 6.12  &       & 6.12  & 6.12  & 18.37 & 8.16  &       & 6.12  & 6.12  & 8.16  & 16.33 &       & 12.24 & 55.10 & 61.22 & 55.10 \\
    \bottomrule
\end{tabular}}
    
\vspace{1em}
\renewcommand{\arraystretch}{1}
\begin{flushleft}
{\bf Panel B: \normalfont $R_{oos}^2$ (\%) for 30 industry portfolios}
\end{flushleft}\vspace{0.1in}
\resizebox{1\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
          & \multicolumn{4}{c}{Univariate} &       & \multicolumn{14}{c}{Multivariate} \\
         \cmidrule{7-20}
          &       &       &       &       &       & \multicolumn{4}{c}{MCMC}      &       & \multicolumn{4}{c}{LVB} &       & \multicolumn{4}{c}{VB} \\
          \cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
          & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} \\
          \midrule
    Mean  & -3.68 & -0.95 & 2.89  & 0.01  &       & -4.13 & -1.23 & 1.22  & 0.06  &       & -30.92 & -0.74 & -0.66 & -0.40 &       & -15.30 & 1.31  & 1.28  & 1.47 \\
    Median   & -3.08 & -0.93 & 3.30  & 0.54  &       & -3.78 & -0.76 & 1.40  & 0.54  &       & -24.24 & -0.56 & -0.58 & -0.80 &       & -9.28 & 1.54  & 1.44  & 1.18 \\
      [1em]
\multicolumn{1}{l}{Percentile} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
     \multicolumn{1}{l}{2.5}   & -14.90 & -10.04 & -3.27 & -8.65 &       & -15.28 & -10.17 & -6.21 & -8.77 &       & -100.17 & -6.08 & -5.77 & -7.44 &       & -68.71 & -3.84 & -4.02 & -3.29 \\
     \multicolumn{1}{l}{25}    & -7.59 & -4.12 & 0.91  & -3.05 &       & -7.43 & -3.94 & -0.72 & -2.61 &       & -40.91 & -2.84 & -2.80 & -2.52 &       & -19.44 & -1.05 & -0.95 & -0.76 \\
     \multicolumn{1}{l}{75}    & 0.95  & 1.64  & 4.74  & 2.77  &       & 0.37  & 1.85  & 3.17  & 2.92  &       & -13.12 & 1.32  & 1.83  & 2.06  &       & -4.66 & 3.40  & 3.11  & 3.58 \\
     \multicolumn{1}{l}{97.5}  & 6.96  & 6.36  & 8.61  & 6.98  &       & 6.69  & 7.49  & 7.93  & 7.77  &       & -2.06 & 4.60  & 4.56  & 6.49  &       & 5.35  & 7.22  & 7.14  & 6.83 \\
 [1em]
    Min   & -15.24 & -10.57 & -3.33 & -8.99 &       & -15.45 & -10.54 & -6.21 & -9.08 &       & -101.64 & -6.27 & -5.93 & -7.62 &       & -75.91 & -3.85 & -4.19 & -3.43 \\
    Max   & 7.06  & 6.55  & 8.78  & 7.11  &       & 6.83  & 7.80  & 8.18  & 8.08  &       & -1.31 & 4.89  & 4.79  & 6.52  &       & 6.43  & 7.48  & 7.54  & 6.83 \\
    $\text{Prob}\left(R_{oos}^2>0\right)$ & 30.00 & 43.33 & 80.00 & 53.33 &       & 30.00 & 43.33 & 63.33 & 56.67 &       & 0.00  & 40.00 & 40.00 & 36.67 &       & 6.67  & 66.67 & 66.67 & 73.33 \\
    \bottomrule
    \end{tabular}%
 }
\label{tab:R2oos_recession}
\end{sidewaystable}

==> Tables/cer.tex <==
\begin{sidewaystable}
\centering
\caption{\bf Certainty equivalent returns}
\vspace{0.1in}
\begin{justify}
\footnotesize{This table reports a set of descriptive statistics for the differential certainty equivalent return expressed in annualised \%. We obtain the certainty equivalent differential by subtracting the average utility of each alternative model $s$, $u_{t,s}$ to the average utility of the historical average forecast, $ u_{t,HA}$. A positive value indicates that a representative investor is willing to pay a positive fee to access the investment strategy implied by a given forecasting model. Panel A reports the results for the 49 industry classification, whereas Panel B reports the results for the 30 industry classification. For each case we report the mean and median $CER$ across industries as well as a set of percentiles and the min and max values. In addition, we report the percentage of industry portfolios for which a given model can generate positive out-of-sample $CER$s, i.e., $\text{Prob}\left(\text{cer}>0\right)$.}
\end{justify}
\vspace{1em}
\renewcommand{\arraystretch}{1}
\centering 
{\bf Panel A: \normalfont Certainty equivalent for the 49 industry portfolios}
\vspace{0.2in}

\resizebox{.9\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
          & \multicolumn{4}{c}{Univariate} &       & \multicolumn{14}{c}{Multivariate} \\
          \cmidrule{7-20}
          &       &       &       &       &       & \multicolumn{4}{c}{MCMC}      &       & \multicolumn{4}{c}{LVB} &       & \multicolumn{4}{c}{VB} \\
          \cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
          & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} \\
          \midrule 
              Mean  & -0.02 & 0.02  & 0.02  & 0.01  &       & -0.02 & 0.00  & 0.02  & 0.00  &       & -0.02 & -0.01 & 0.00  & -0.01 &       & -0.04 & 0.00  & 0.00  & -0.02 \\
    Median & -0.03 & 0.04  & 0.05  & 0.02  &       & -0.03 & -0.01 & -0.02 & 0.01  &       & -0.01 & -0.05 & -0.05 & -0.05 &       & -0.01 & 0.02  & 0.05  & 0.04 \\
    Multiasset & 0.01  & 0.15  & 0.31  & 0.16  &       & -0.04 & 0.42  & 0.67  & 0.33  &       & 0.38  & 0.39  & 0.54  & 0.67  &       & -0.36 & 0.63  & 0.26  & 0.85 \\
   [1em]
\multicolumn{1}{l}{Percentile} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
  \multicolumn{1}{l}{2.5}    & -1.40 & -1.20 & -0.79 & -1.05 &       & -1.63 & -1.10 & -0.52 & -0.94 &       & -1.27 & -0.86 & -0.87 & -0.55 &       & -1.67 & -0.83 & -0.99 & -1.34 \\
   \multicolumn{1}{l}{25}     & -0.30 & -0.16 & -0.07 & -0.23 &       & -0.28 & -0.24 & -0.13 & -0.22 &       & -0.39 & -0.27 & -0.27 & -0.16 &       & -0.34 & -0.26 & -0.20 & -0.30 \\
    \multicolumn{1}{l}{75}     & 0.26  & 0.38  & 0.28  & 0.29  &       & 0.27  & 0.29  & 0.22  & 0.22  &       & 0.28  & 0.29  & 0.25  & 0.19  &       & 0.31  & 0.26  & 0.23  & 0.19 \\
    \multicolumn{1}{l}{97.5}  & 0.31  & 0.36  & 0.44  & 0.78  &       & 0.37  & 0.77  & 0.46  & 0.72  &       & 0.56  & 0.77  & 0.97  & 0.55  &       & 0.23  & 0.70  & 0.81  & 1.15 \\
[1em]
    Min   & -1.61 & -1.98 & -1.28 & -1.39 &       & -1.84 & -1.38 & -0.66 & -1.17 &       & -1.39 & -0.91 & -1.05 & -0.85 &       & -1.74 & -1.33 & -1.60 & -1.46 \\
    Max   & 0.34  & 0.45  & 0.46  & 0.83  &       & 1.21  & 0.90  & 0.54  & 0.81  &       & 0.76  & 0.97  & 1.14  & 0.67  &       & 0.44  & 0.89  & 0.95  & 1.44 \\
    $\text{Prob}\left(\text{cer}>0\right)$ & 33.98 & 50.14 & 51.18 & 52.14 &       & 44.90 & 48.98 & 41.02 & 51.10 &       & 48.98 & 48.98 & 43.06 & 42.86 &       & 46.94 & 53.06 & 55.10 & 55.10 \\
    \bottomrule
\end{tabular}}
    
\vspace{1em}
\renewcommand{\arraystretch}{1}
\centering 
{\bf Panel B: \normalfont Certainty equivalent for the 30 industry portfolios}
\vspace{0.2in}

\resizebox{.9\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
          & \multicolumn{4}{c}{Univariate} &       & \multicolumn{14}{c}{Multivariate} \\
         \cmidrule{7-20}
          &       &       &       &       &       & \multicolumn{4}{c}{MCMC}      &       & \multicolumn{4}{c}{LVB} &       & \multicolumn{4}{c}{VB} \\
          \cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
          & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} &       & \multicolumn{1}{c}{Normal} & \multicolumn{1}{c}{BL} & \multicolumn{1}{c}{NG} & \multicolumn{1}{c}{HS} \\
          \midrule 
        Mean  & 0.00  & 0.01  & 0.00  & 0.01  &       & 0.00  & 0.01  & 0.01  & 0.01  &       & -0.15 & -0.01 & -0.01 & 0.00  &       & -0.10 & 0.00  & 0.00  & 0.01 \\
    Median & -0.01 & -0.01 & -0.02 & -0.02 &       & -0.02 & 0.00  & 0.01  & -0.01 &       & -0.12 & -0.01 & -0.01 & -0.02 &       & -0.04 & 0.01  & 0.01  & 0.01 \\
    Multiasset & 0.13  & 0.48  & 0.15  & 0.44  &       & 0.16  & 0.48  & 0.32  & 0.40  &       & -0.20 & 0.04  & 0.05  & 0.08  &       & 0.36  & 0.38  & 0.38  & 0.49 \\
  [1em]
\multicolumn{1}{l}{Percentile} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{l}{2.5}   & -0.41 & -0.25 & -0.11 & -0.21 &       & -0.38 & -0.29 & -0.13 & -0.21 &       & -0.92 & -0.23 & -0.24 & -0.23 &       & -0.96 & -0.25 & -0.24 & -0.20 \\
   \multicolumn{1}{l}{25}    & -0.07 & -0.05 & -0.06 & -0.05 &       & -0.08 & -0.08 & -0.05 & -0.06 &       & -0.30 & -0.09 & -0.09 & -0.08 &       & -0.32 & -0.05 & -0.06 & -0.05 \\
    \multicolumn{1}{l}{75}    & 0.06  & 0.05  & 0.06  & 0.07  &       & 0.05  & 0.07  & 0.07  & 0.06  &       & 0.05  & 0.05  & 0.07  & 0.08  &       & 0.15  & 0.06  & 0.05  & 0.06 \\
    \multicolumn{1}{l}{97.5}  & 0.12  & 0.36  & 0.17  & 0.36  &       & 0.26  & 0.34  & 0.20  & 0.28  &       & 0.26  & 0.31  & 0.27  & 0.21  &       & 0.37  & 0.24  & 0.23  & 0.20 \\
[1em]
    Min   & -0.48 & -0.29 & -0.11 & -0.22 &       & -0.41 & -0.31 & -0.14 & -0.23 &       & -0.95 & -0.24 & -0.26 & -0.24 &       & -1.09 & -0.27 & -0.26 & -0.22 \\
    Max   & 0.16  & 0.38  & 0.19  & 0.37  &       & 0.44  & 0.35  & 0.20  & 0.28  &       & 0.34  & 0.37  & 0.31  & 0.59  &       & 0.40  & 0.53  & 0.44  & 0.76 \\
    $\text{Prob}\left(\text{cer}>0\right)$ & 40.00 & 46.67 & 46.67 & 40.00 &       & 46.67 & 50.00 & 50.00 & 46.67 &       & 33.33 & 50.00 & 50.00 & 43.33 &       & 46.67 & 56.67 & 56.67 & 56.67 \\
    \bottomrule
    \end{tabular}%
 }
\label{tab:cer}
\end{sidewaystable}
